Sampling and Remote Estimation for the Ornstein-Uhlenbeck Process through Queues: Age of Information and Beyond

The age of information, as a metric for evaluating information freshness, has received a lot of attention. Recently, an interesting connection between the age of information and remote estimation error was found in a sampling problem of Wiener processes: If the sampler has no knowledge of the signal being sampled, the optimal sampling strategy is to minimize the age of information; however, by exploiting causal knowledge of the signal values, it is possible to achieve a smaller estimation error. In this paper, we extend a previous study by investigating a problem of sampling a stationary Gauss-Markov process, namely the Ornstein-Uhlenbeck (OU) process. The optimal sampling problem is formulated as a constrained continuous-time Markov decision process (MDP) with an uncountable state space. We provide an exact solution to this MDP: The optimal sampling policy is a threshold policy on instantaneous estimation error and the threshold is found. Further, if the sampler has no knowledge of the OU process, the optimal sampling problem reduces to an MDP for minimizing a nonlinear age of information metric. The age-optimal sampling policy is a threshold policy on expected estimation error and the threshold is found. These results hold for (i) general service time distributions of the queueing server and (ii) sampling problems both with and without a sampling rate constraint. Numerical results are provided to compare different sampling policies.

==> abstract.tex <==
\begin{abstract}
%In this paper, we investigate a problem of sampling an Ornstein-Uhlenbeck (OU) process, which is the continuous-time analogue of the discrete-time AR(1) process.
%Samples of the OU process are forwarded through a queue to a remote estimator, which estimates the real-time value of the OU process from causally received samples.
%The optimal sampling problem for minimizing the mean-squared estimation error under a sampling rate constraint is formulated as a constrained continuous-time Markov decision process (MDP) with an uncountable state space. We provide an exact solution to this MDP: The optimal sampling policy is a threshold policy on \emph{instantaneous} estimation error, and the threshold is characterized based on the optimal objective value of the MDP and the sampling rate constraint. Further, we consider a class of signal-ignorant sampling policies, where the sampling times are determined without using knowledge of the observed OU process. 
%The optimal signal-ignorant sampler design problem is equivalent to an MDP  for minimizing a nonlinear age of information metric, which has been solved recently. We find that the optimal signal-ignorant sampling policy is a threshold policy on \emph{expected} estimation error, and the threshold is determined in a similar fashion as mentioned above. These optimal sampling results hold for general service time distributions of the queueing server. 
%Numerical results are provided to compare different sampling policies. 
\ignore{In this paper, we investigate a problem of sampling a stationary Gauss-Markov process, namely the Ornstein-Uhlenbeck (OU) process, which is the continuous-time analogue of the discrete-time AR(1) process. Samples of the OU process are forwarded to a remote estimator through a queue.  
The optimal sampling problem for minimizing the mean-squared estimation error under a sampling rate constraint is formulated as a constrained continuous-time Markov decision process (MDP) with an uncountable state space. We provide an exact solution to this MDP: The optimal sampling policy is a threshold policy on \emph{instantaneous} estimation error, and the threshold is characterized based on the optimal objective value of the MDP and the sampling rate constraint. If the sampling times are determined without using knowledge  of the observed OU process, the optimal sampling problem reduces to an MDP for minimizing a nonlinear age of information metric. This reveals a relationship between  remote estimation and nonlinear age metrics. The age-optimal sampling policy is a threshold policy on \emph{expected} estimation error, and the threshold is determined by the optimal objective value and the sampling rate constraint. These optimal sampling policies can be computed by bisection search, and the curse of dimensionality is circumvented. These results hold for general service time distributions of the queueing server. Numerical results are provided to compare different sampling policies. 
The age of information, as a metric for evaluating information freshness, has received a lot of attention. 
Recently, an interesting connection between the age of information and remote estimation error was found in a sampling problem of Wiener processes: If the sampler has no knowledge of the signal being sampled,  the optimal sampling strategy is to minimize the age of information; however, by exploiting causal knowledge of the signal values, it is possible to achieve a smaller estimation error. 
In this paper, we extend previous study by investigating a problem of sampling a stationary Gauss-Markov process, namely the Ornstein-Uhlenbeck (OU) process.
%, which is the continuous-time analogue of the discrete-time AR(1) process.
The optimal sampling problem
is formulated as a constrained continuous-time Markov decision process (MDP) with an uncountable state space. We provide an exact solution to this MDP: The optimal sampling policy is a threshold policy on \emph{instantaneous estimation error} and the threshold is found. Further, if the sampler has no knowledge of the  OU process, the optimal sampling problem reduces to an MDP for minimizing a \emph{nonlinear} age of information metric. The age-optimal sampling policy is a threshold policy on \emph{expected estimation error} and the threshold is found.  These results hold for (i) general service time distributions of the queueing server and (ii) sampling problems both with and without a sampling rate constraint. Numerical results are provided to compare different sampling policies.}
%The age of information, as a metric for evaluating information freshness, has received a lot of attention. 
Recently, a connection between the age of information and remote estimation error was found in a sampling problem of Wiener processes: If the sampler has no knowledge of the signal being sampled,  the optimal sampling strategy is to minimize the age of information; however, by exploiting causal knowledge of the signal values, it is possible to achieve a smaller estimation error. 
In this paper, we generalize the previous study by investigating a problem of sampling a stationary Gauss-Markov process named the Ornstein-Uhlenbeck (OU) process, where we aim to find useful insights for solving the problems of sampling more general signals. 
%, which is the continuous-time analogue of the discrete-time AR(1) process.
The optimal sampling problem is formulated as a constrained continuous-time Markov decision process (MDP) with an uncountable state space. We provide an exact solution to this MDP: The optimal sampling policy is a threshold policy on \emph{instantaneous estimation error} and the threshold is found. Further, if the sampler has no knowledge of the OU process, the optimal sampling problem reduces to an MDP for minimizing a \emph{nonlinear} age of information metric. The age-optimal sampling policy is a threshold policy on \emph{expected estimation error} and the threshold is found. In both problems, the optimal sampling policies can be computed by bisection search, and the curse of dimensionality is circumvented. These results hold for (i) general service time distributions of the queueing server and (ii) sampling problems both with and without a sampling rate constraint. 
Numerical results are provided to compare different sampling policies.
\end{abstract}
